Multiple Concurrent Proposers: Why and How

Traditional single-proposer blockchains suffer from miner extractable value (MEV), where validators exploit their serial monopoly on transaction inclusion and ordering to extract rents from users. While there have been many developments at the application layer to reduce the impact of MEV, these approaches largely require auctions as a subcomponent. Running auctions efficiently on chain requires two key properties of the underlying consensus protocol: selective-censorship resistance and hiding. These properties guarantee that an adversary can neither selectively delay transactions nor see their contents before they are confirmed. We propose a multiple concurrent proposer (MCP) protocol offering exactly these properties.

==> lib/defer.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\RequirePackage{expl3}
\RequirePackage{scontents}


%
%
%
\ExplSyntaxOn

%
%
%
\cs_new_protected:Npn \defer_new_group:nn #1 #2 {
  %
  \bool_if_exist:cF { l__defer_#1 _bool } { \bool_new:c { l__defer_#1 _bool } }
  %
  \tl_set:Nx \l_tmpa_tl { \tl_lower_case:n {#2} }
  %
  \str_if_eq:VnTF \l_tmpa_tl {deferred}
    { \bool_set_true:c  { l__defer_#1 _bool } }
    { \bool_set_false:c { l__defer_#1 _bool } }
}


%
%
%

%
%
\NewDocumentCommand{\newdefergroup}{m O{deferred}}{
  \defer_new_group:nn {#1}{#2}
}

%
%
\NewDocumentEnvironment{ifdeferred}{m +b}{%
  \bool_if:cT { l__defer_#1 _bool } { #2 }%
}{}

%
%
\NewDocumentEnvironment{ifnotdeferred}{m +b}{%
  \bool_if:cF { l__defer_#1 _bool } { #2 }%
}{}

%
%
%
\NewDocumentEnvironment{defer}{m +b}{%
  \bool_if:cTF { l__defer_#1 _bool }{%
    %
    \Scontents[store-cmd=defer@#1,print-cmd=false]{#2}%
  }{%
    %
    #2%
  }%
}{}

%
%
\NewDocumentCommand{\printdefergroup}{m}{%
  %
  \foreachsc{defer@#1}%
}

\ExplSyntaxOff

%
%
%

%
%
%
%
\NewDocumentCommand{\deferredproof}{m m}{%
  \begin{ifdeferred}{#1}%
    Proof of \cref{#2} is deferred to \cref{sec:deferred-#1}.%
  \end{ifdeferred}%
}

%
%
%
\NewDocumentCommand{\deferredsection}{m m}{%
  \begin{ifdeferred}{#1}%
    \section{#2}%
    \label{sec:deferred-#1}%
    \printdefergroup{#1}%
  \end{ifdeferred}%
}

